Sensitivity analysis for publication bias on the time-dependent summary ROC analysis in meta-analysis of prognosis studies

In the analysis of prognosis studies with time-to-event outcomes, dichotomization of patients is often made. As the evaluations of prognostic capacity, the survivals of groups with high/low expression of the biomarker are often estimated by the Kaplan-Meier method, and the difference between groups is summarized via the hazard ratio (HR). The high/low expressions are usually determined by study-specific cutoff values, which brings heterogeneity over multiple prognosis studies and difficulty to synthesizing the results in a simple way. In meta-analysis of diagnostic studies with binary outcomes, the summary receiver operating characteristics (SROC) analysis provides a useful cutoff-free summary over studies. Recently, this methodology has been extended to the time-dependent SROC analysis for time-to-event outcomes in meta-analysis of prognosis studies. In this paper, we propose a sensitivity analysis method for evaluating the impact of publication bias on the time-dependent SROC analysis. Our proposal extends the recently introduced sensitivity analysis method for meta-analysis of diagnostic studies based on the bivariate normal model on sensitivity and specificity pairs. To model the selective publication process specific to prognosis studies, we introduce a trivariate model on the time-dependent sensitivity and specificity and the log-transformed HR. Based on the proved asymptotic property of the trivariate model, we introduce a likelihood based sensitivity analysis method based on the conditional likelihood constrained by the expected proportion of published studies. We illustrate the proposed sensitivity analysis method through the meta-analysis of Ki67 for breast cancer. Simulation studies are conducted to evaluate the performance of the proposed method.

==> tab/tb-conf.tex <==
% \begin{table}[!tbh]
% \centering
% \caption{Notations for cell frequencies in 2 × 2 confusion matrix for diagnostic study $i$.}
% \label{tab:confusion-1}
% \begin{tabular}{ccccc}
% \toprule
%  &  & \multicolumn{2}{c}{True disease status} &  \\ \midrule
%  &  & $D=0$ & $D=1$ &  \\ \midrule
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Biomarker \\ expression\end{tabular}} & $Z=0:\tilde X\le v^{(i)}$ & $n_{00}^{(i)}$ & $n_{01}^{(i)}$ & $n_0^{(i)}$ \\ \cmidrule{2-5} 
%  & $Z=1:\tilde X> v^{(i)}$ & $n_{10}^{(i)}$ & $n_{11}^{(i)}$ & $n_1^{(i)}$ \\ \midrule
%  &  & $n_{+0}^{(i)}$ & $n_{+1}^{(i)}$ & $n^{(i)}$ \\ \bottomrule
% \end{tabular}
% \begin{tablenotes}
% \item 
% All the cells are observable.
% \end{tablenotes}
% \end{table}



\begin{table}[!tbh]
\centering
\caption{Notations for cell frequencies in 2 × 2 confusion matrix for prognostic study $i$.}
\label{tab:confusion}
\begin{tabular}{ccccc}
\toprule
 &  & \multicolumn{2}{c}{True disease status} &  \\ \midrule
 &  & $D(t)=0:\tilde T\le t$ & $D(t)=1:\tilde T> t$ &  \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Biomarker \\ expression\end{tabular}} & $Z=0:\tilde X\le v^{(i)}$ & $N_{00}^{(i)}$ & $N_{01}^{(i)}$ & $n_0^{(i)}$ \\ \cmidrule{2-5} 
 & $Z=1:\tilde X> v^{(i)}$ & $N_{10}^{(i)}$ & $N_{11}^{(i)}$ & $n_1^{(i)}$ \\ \midrule
 &  & $N_{+0}^{(i)}$ & $N_{+1}^{(i)}$ & $n^{(i)}$ \\ \bottomrule
\end{tabular}
\begin{tablenotes}
\item 
            Only $n_{0}^{(i)}, n_{1}^{(i)}, n^{(i)}$ are observable, the otherwise are unobservable.
\end{tablenotes}
\end{table}
